Learning Graphical Models from a Distributed Stream

A current challenge for data management systems is to support the construction and maintenance of machine learning models over data that is large, multi-dimensional, and evolving. While systems that could support these tasks are emerging, the need to scale to distributed, streaming data requires new models and algorithms. In this setting, as well as computational scalability and model accuracy, we also need to minimize the amount of communication between distributed processors, which is the chief component of latency. We study Bayesian networks, the workhorse of graphical models, and present a communication-efficient method for continuously learning and maintaining a Bayesian network model over data that is arriving as a distributed stream partitioned across multiple processors. We show a strategy for maintaining model parameters that leads to an exponential reduction in communication when compared with baseline approaches to maintain the exact MLE (maximum likelihood estimation). Meanwhile, our strategy provides similar prediction errors for the target distribution and for classification tasks.

==> classification.tex <==
%-----------------------
\section{Classification}
\label{sec:class}
%-----------------------
In the previous section, our objective is to guarantee the accuracy of the joint probability distribution, which satisfies the probability query. Another important task is to do the classification on the \bayesnet, which is to find the most likely assignment to some subset of variables given some evidence. More precisely, given the evidence $e$, the objective of classification is to find the most likely assignment to subset variables $\bm{Y}$:
\[
Class(\bm{Y} \mid e) = \argmax_y \prob{y,e}
\]

%----------------------
\begin{definition}
\label{defn:class-obj}
Given a \bayesnet $\mathcal{G}$, let $Y$ denote the set of variables need to assigned. For any evidence $e$, our objective is
\[
\empProb{Y=b \mid e} \ge (1-\eps) \cdot \max_i \empProb{Y=i \mid e}
\] 
where $\eps$ is the approximation factor.  
\end{definition}
In other words, we want to find the assignment of interested set of variables $Y$ with conditional probability close to the maximum probability, if not equal to the maximum.
%----------------------

%----------------------
\begin{lemma}
\label{lem:subset-vars}
If for all the variables $\mathcal{X}$, we have 
\[
e^{-\eps} \leq \frac{\empProb{\mathcal{X}}}{\estProb{\mathcal{X}}} \leq e^{\eps}
\]
Then for any subset of non-overlapping variables $\bm{X}$ and $\bm{Y}$, $\bm{X} \cup \bm{Y} = \emptyset$,
\[
e^{-\eps} \leq \frac{\empProb{\bm{Y} \mid \bm{X}}}{\estProb{\bm{Y} \mid \bm{X}}} \leq e^{\eps}
\]
\end{lemma}
\begin{proof}

\end{proof}
%----------------------


%----------------------
\begin{lemma}
\label{lem:classification}
When the following is true
\[
e^{-\eps / 2} \leq \frac{\empProb{\mathcal{X}}}{\estProb{\mathcal{X}}} \leq e^{\eps / 2}
\]
given evidence $e$ and set of variables $Y$, we can find assignment $\bm{b}$ such that 
\[
\empProb{\bm{Y}=\bm{b} \mid e} \ge (1-\eps) \cdot \max_i \empProb{Y=i \mid e}
\]  
\end{lemma}
%----------------------
\begin{proof}
From Lemma~\ref{lem:subset-vars}, for assignment $\bm{b}$, we have
\[
e^{\eps/2} \cdot \empProb{\bm{Y}=\bm{b} \mid e} \geq \estProb{\bm{Y}=\bm{b} \mid e}
\]
Let $\bm{b}^* = \argmax_i \empProb{Y=i \mid e}$, when using the approximate counters, as $\bm{b}$ is the most like assignment,
\[
\estProb{\bm{Y}=\bm{b} \mid e} \geq \estProb{\bm{Y}=\bm{b}^* \mid e}
\]
From Lemma~\ref{lem:subset-vars},for assignment $\bm{b}^*$, we have
\[
\estProb{\bm{Y}=\bm{b}^* \mid e} \geq e^{-\eps/2} \cdot \empProb{\bm{Y}=\bm{b}^* \mid e}
\]
So we can derive that
\[
\empProb{\bm{Y}=\bm{b} \mid e} \geq e^{-\eps} \cdot \empProb{\bm{Y}=\bm{b}^* \mid e}
\]
\end{proof}

==> naivebayes.tex <==
%------------------------------------------------
\section{Algorithm for Approximate Na{\"i}ve Bayes}
\label{sec:naivebayes}
%----------------------------------------------
Consider \naivebayes problem in a distributed system, it maybe expensive, both in terms of communication as well as computation, to find the label which exactly maximizes the posterior probability. Hence we consider the following approximate version of the Bayesian classification problem.

%------------------
\begin{definition}
\label{defn:abc}
Given an input vector $X$ and approximation parameter $0 < \eps < 1$, the $\eps$-Approximate Bayesian Classifier (ABC) assigns a label $\ell$ such that 
\begin{equation}
\label{eqn:abc-dfn}
\empCp{Y=\ell}{X} \ge (1-\eps) \cdot \max_k \empCp{Y=k}{X}
\end{equation}
\end{definition}
%------------------
In other words, the classifier returns a label whose posterior probability is very close to the label with the maximum probability, if not equal to the maximum.


\remove{
%----------------------------------
\subsection{Parameters to Estimate}
%----------------------------------
There are two sets of parameters to estimate: 
(1)~the probabilities $\Pr(Y=k)$ for each class $k = 1 \ldots K$, and
(2)~the conditional probabilities $\cp{X_i=j}{Y=k}$ for each dimension $i=1\ldots d$, each possible $j = 1\ldots J$, and each possible label $k=1\ldots K$. There are $dJK$ such parameters. 

The classifier estimates these parameters through their empirical counts in the training data. We use the notation $\D{\gamma}$ to denote the number of instances in the training data $D$ that satisfies property $\gamma$. Let $\theta_{ijk}$ denote $\cp{X_i=j}{Y=k}$ and $\pi_k$ denote $\Pr(Y=k)$. To estimate $\theta_{ijk}$ and $\pi_k$, we keep three sets of counters:
(1) $\xctr_{ijk} = \D{X_i=j, Y=k}$, 
(2) $\yctr_k  = \D{Y=k}$ and 
(3) $\yctr$, the number of training instances.
Let $\tilde{\theta}_{ijk}$ denote an estimate of $\theta_{ijk}$ and $\tilde{\pi}_k$ an estimate of $\pi_k$. We have
 
\[
\tilde{\theta}_{ijk} = \frac{\xctr_{ijk}}{\yctr_k}  \quad
\tilde{\pi}_k = \frac{\yctr_k}{\yctr}
\]

Then the estimated most probable value of class $Y$ is
\begin{align*}
Y & = \argmax_k \left( \frac{\yctr_k}{\yctr} \cdot \prod_{i=1}^d \frac{\xctr_{ijk}}{\yctr_k} \right)  \\
& = \argmax_k \left( \frac{1}{\yctr_k^{d-1}} \cdot \prod_{i=1}^d \xctr_{ijk} \right)
\end{align*}
}


%---------------------------------------------
\subsection{Approximate Na{\"i}ve Bayes Algorithm}
%---------------------------------------------
The algorithm for ABC maintains multiple distributed counters, one for each parameter in the factorized Equation~\ref{eqn:naivebayes}. Let $C$ denote the total number of training instances in the system. For $1 \le k \le K$, let $C_k$ denote the number of instances with label $k$. For $1 \le i \le d$, $1 \le j \le J$, and $1 \le k \le K$, let $C_{ijk}$ denote the number of events where $X_i = j$ and the class label is $k$. We use $DistCounter$ as subroutine to maintain these counters. $\dc_k$ and $\dc_{ijk}$ are the distributed counters that approximately track $C_k$ and $C_{ijk}$ respectively. The distributed counter provides a method called $value$ which returns the value of the counter and is approximately correct. Initialization, maintenance, and query are presented in Algorithms~\ref{algo:ABC2-init}, \ref{algo:ABC2-train}, and \ref{algo:ABC2-test} respectively.

%We improve our algorithm stated in Section~\ref{sec:abc-algorithm1} to achieve better communication cost. Initialization, maintenance, and query are presented in Algorithms~\ref{algo:ABC2-init}, \ref{algo:ABC2-train}, and \ref{algo:ABC2-test} respectively.

%----------------------------
\begin{algorithm}
\label{algo:ABC2-init}
\DontPrintSemicolon
\caption{ABCInit($\eps, \delta, d, J, K, p$)}
\ForEach{$k$ from $1$ to $K$} {
	$\dc_k \gets$ DistCounter$\left(p, \frac{\eps}{10d}, \delta \right)$ \;
	\ForEach{$i$ from $1$ to $d$, and $j$ from $1$ to $J$} 
	{$\dc_{ijk} \gets$ DistCounter$\left(p, \frac{\eps}{16\sqrt{d}}\right)$\;}
}
\end{algorithm}
%----------------------------

%----------------------------
\begin{algorithm}
\DontPrintSemicolon
\label{algo:ABC2-train}
\caption{ABCUpdate$(\alpha, \ell)$}
\KwIn{$\alpha=\langle \alpha_1, \ldots, \alpha_d \rangle$ is an observation; $\ell$ is a label}
Increment $\dc_{\ell}$ \;
\ForEach{$i$ from $1$ to $d$} 
{Increment $\dc_{i, \alpha_i, \ell}$}
\end{algorithm}
%----------------------------

%----------------------------
\begin{algorithm}
\label{algo:ABC2-test}
\DontPrintSemicolon
\caption{ABCQuery($\alpha$)}
\KwIn{$\alpha=\langle \alpha_1, \alpha_2, \ldots, \alpha_d \rangle$ is an input vector to be labeled}
\KwOut{Class label for input $\alpha$}
\ForEach{$k$ from $1$ to $K$}
{
	$q_k \gets \dc_k.value() $  \;
	\ForEach{$i$ from $1$ to $d$}
	{
		$q_k \gets q_k * \frac{\dc_{i, \alpha_i, k}.value()}{\dc_k.value()}$   \;
	}
}
\Return $\argmax_{k} q_k$  \;
 \end{algorithm}
%----------------------------


%----------------------------------
\begin{theorem}
\label{theo:ABC2-perf}
Given approximation factor $\eps$ and error probability $\delta$ where $0 < \eps < 1/4$, and $0 < \delta < 1$, the distributed algorithm presented in Algorithms~\ref{algo:ABC2-init}, \ref{algo:ABC2-train}, and \ref{algo:ABC2-test} is a \naivebayes classifier, when presented with input $X=\alpha$, returns a label $\ell$ that obeys the ABC guarantee (Definition~\ref{defn:abc}) with probability at least $7/8$. The total communication cost across processing all updates in Algorithm ABCUpdate is $O \left( \frac{\sqrt{p}d^{3/2}JK}{\eps} \log C^{max} \right)$ bits, where $C^{max}$ is the total number of training instances. The space used at each local site is $O(dJK \log C^{max})$ bits and amortized processing time per update is $O(1)$.
\end{theorem}
%----------------------------------

\begin{proof}
Given input $\alpha$, let $\ell$ be the label returned by Algorithm~ABCQuery$(\alpha)$.
Our goal is to prove that\footnote{Note that the probabilities in the next two equations are empirical probabilities. These two need to be clearly differentiated from the probabilities resulting from explicit randomization, which appear later.}
\begin{equation}
\label{eqn:ABC2-1}
\empCp{Y=\ell}{X=\alpha} \ge ( 1- \eps) \cdot \max_k\empCp{Y=k}{X=\alpha}
\end{equation}
%---------------------

Note that for any $k$,
\begin{equation}
\label{eqn:ABC2-2}
\cp{Y=k}{X=\alpha} = \frac{\prob{Y=k} \cdot \prod_{i=1}^d \cp{X_i=\alpha_i}{Y=k}}{\sum_{l=1}^K \prob{Y=l} \cdot \cp{X}{Y=l}}
\end{equation} 

%Let $C_k$ and $C_{i\alpha_ik}$ as defined in Section~\ref{sec:algorithm}. Recall that $C_k$ is the number of instances with label $k$, $C_{i\alpha_ik}$ is number of instances that $X_i=\alpha_i$ and label is $k$. 
Let $Q(k,\alpha)$ be defined as:
\begin{equation}
\label{eqn:ABC2-3}
Q(k,\alpha) = C_k \cdot \prod_{i=1}^d \frac{C_{i\alpha_ik}}{C_k}
\end{equation}

$Q(k,\alpha)$ is proportional to the numerator of $\cp{Y=k}{X=\alpha}$. We note that Equation~\ref{eqn:ABC2-1} is equivalent to the following equation \ref{eqn:ABC2-4}, and our goal henceforth is to show that Equation~\ref{eqn:ABC2-4} holds with high probability.
\begin{equation}
\label{eqn:ABC2-4}
Q(\ell,\alpha) \ge ( 1- \eps) \cdot \max_k Q(k,\alpha)
\end{equation}
%---------------------

Let $\tilde{C}_k$ and $\tilde{C}_{i\alpha_ik}$ be the values of $\dc_k$ and $\dc_{ijk}$ when queried by Algorithm~ABCQuery. 
$\tilde{C}_k$ and $\tilde{C}_{i\alpha_ik}$ are estimators of ${C}_k$ and ${C}_{i\alpha_ik}$, respectively.
For each $1 \le k \le K$, we define 
\begin{equation}
\label{eqn:ABC2-6}
\tilde{Q}(k,\alpha)= \tilde{C}_k \cdot \prod_{i=1}^d \frac{\tilde{C}_{i\alpha_ik}}{\tilde{C}_k}
\end{equation}
Given input $\alpha$, the Algorithm~ABCQuery($\alpha$) returns label $\ell$ that maximizes $\tilde{Q}(\ell, \alpha)$.
%--------------------- 

We can derive $\tilde{Q}(k,\alpha) / Q(k,\alpha)$ in the following form:
\begin{align*}
\frac{\tilde{Q}(k,\alpha)}{Q(k,\alpha)} & = \frac{\tilde{C}_k}{C_k}  \cdot \prod_{i=1}^d \frac{\tilde{C}_{i\alpha_ik}}{C_{i\alpha_ik}} \cdot \frac{C_k}{\tilde{C}_k}   \\
& = \left( \frac{C_k}{\tilde{C}_k} \right)^{d-1} \cdot \prod_{i=1}^d \frac{\tilde{C}_{i\alpha_ik}}{C_{i\alpha_ik}} \\
\end{align*}
%---------------------

From the approximation factors we set in Algorithm~\ref{algo:ABC2-init}, and using Lemma~\ref{lem:rctr-1}, we have with high probability 
%-----------------
\begin{equation}
\label{eqn:ABC2-5}
\begin{aligned}
\left( 1-\frac{\eps}{10d} \right) C_k \leq \tilde{C}_k \leq \left( 1+\frac{\eps}{10d} \right)C_k  \\
%\left( 1-\frac{\eps}{16\sqrt{d}} \right) C_{i\alpha_ik} \leq \tilde{C}_{i\alpha_ik}  \leq  \left( 1+\frac{\eps}{16\sqrt{d}} \right) C_{i\alpha_ik}  \\
\end{aligned}
\end{equation}
%-----------------

{\color{red} Some work is needed to get the probabilities right, but this should be minor.}

%-----------------------------------
From Lemma~\ref{lem:rctr-1} we have:
\[
\expec{\tilde{C}_{i\alpha_ik}} = C_{i\alpha_ik}  \quad
\variance{\tilde{C}_{i\alpha_ik}} \leq \left( \frac{\eps}{16\sqrt{d}} \right)^2 \cdot C_{i\alpha_ik}^2
\]
%-----------------------------------

So we can derive that
\[
\expec{\tilde{C}_{i\alpha_ik}^2} = \variance{\tilde{C}_{i\alpha_ik}} + \left( \expec{\tilde{C}_{i\alpha_ik}} \right)^2 
\leq \left( 1+\frac{\eps^2}{256d} \right) \cdot C_{i\alpha_ik}^2
\]

Define $F=\prod_{i=1}^d \tilde{C}_{i\alpha_ik}$, $f=\prod_{i=1}^d C_{i\alpha_ik}$. Based on the independence of $\tilde{C}_{i\alpha_ik}$, we have
\begin{align*}
\variance{F} & = \expec{F^2} - \left( \expec{F} \right)^2  \\
& = \prod_{i=1}^d \expec{\tilde{C}_{i\alpha_ik}^2} - \prod_{i=1}^d \left( \expec{\tilde{C}_{i\alpha_ik}} \right)^2  \\
& \leq f^2 \cdot \prod_{i=1}^d \left( 1+\frac{\eps^2}{256d}\right)  - f^2 \\
& \leq f^2 \cdot \left( e^{\eps^2/256} - 1 \right)  \\
\end{align*}

Apply the fact that $e^x < 1+2x$ when $0<x<\frac{1}{e}$,
\[
\variance{F} \leq f^2 \cdot \left( 1+2 \cdot \frac{\eps^2}{256} -1 \right) = \frac{\eps^2 f^2}{128}
\]

Based on Chebyshev's inequality
\[
\prob{\left| F-\expec{F} \right| \geq \frac{\eps f}{4}} \leq \frac{16 \cdot \variance{F}}{\eps^2 f^2} \leq \frac{1}{8}
\]

As $\expec{F} = f$, we have
\[
\prob{|F-f| \geq \frac{\eps f}{4}} \leq \frac{1}{8} 
\]
So with high probability at least $7/8$,
\begin{equation}
\label{eqn:ABC2-7}
1-\frac{\eps}{4} \leq \prod_{i=1}^d \frac{\tilde{C}_{i\alpha_ik}}{C_{i\alpha_ik}} \leq 1+\frac{\eps}{4}
\end{equation}
%---------------------


From Equation~\ref{eqn:ABC2-5}, we have
\begin{equation}
\label{eqn:ABC2-8}
\frac{\tilde{C}_k}{C_k} \leq 1 + \frac{\eps}{10d} \quad \text{and} \quad
\frac{C_k}{\tilde{C}_k} < \frac{1}{1-\frac{\eps}{10d}} < 1 + \frac{\eps}{9d} 
\end{equation}

From Equation~\ref{eqn:ABC2-8},
\begin{equation}
\left( \frac{C_k}{\tilde{C}_k} \right)^{d-1} < \left( 1 + \frac{\eps}{9d} \right)^{d-1} < e^{\eps/9} < 1 + \frac{2 \eps}{9}    
\end{equation}

On the other hand, 
\[
\left( \frac{\tilde{C}_k}{C_k} \right)^{d-1} \leq \left( 1 + \frac{\eps}{10d} \right)^{d-1} < e^{\eps/10} < 1+\frac{\eps}{5}
\]

So we have
\begin{equation}
\label{eqn:ABC2-9}
1-\frac{\eps}{5} < \left( \frac{C_k}{\tilde{C}_k} \right)^{d-1} < 1 + \frac{2 \eps}{9}  
\end{equation}

Combine Equation~\ref{eqn:ABC2-7} and \ref{eqn:ABC2-9}
\begin{equation}
\label{eqn:ABC2-10}
1- \frac{\eps}{2} < \frac{\tilde{Q}(k,\alpha)}{Q(k,\alpha)} < 1 + \frac{\eps}{2}
\end{equation}


%---------------------------
Let $\ell^*=\argmax_k Q(k,\alpha)$, through Equation\ref{eqn:ABC2-10}
\begin{align*}
\tilde{Q}(\ell,\alpha) \leq (1+\eps/2)Q(\ell,\alpha) \\
\tilde{Q}(\ell^*,\alpha) \geq (1-\eps/2)Q(\ell^*,\alpha) 
\end{align*}
As $\ell$ is the return label by ABCQuery, $\tilde{Q}(\ell,\alpha) \geq \tilde{Q}(\ell^*,\alpha)$
\begin{equation}
\label{eqn:ABC2-11}
Q(\ell,\alpha) \geq \frac{1-\eps/2}{1+\eps/2} \cdot Q(\ell^*,\alpha) > (1-\eps)\cdot Q(\ell^*,\alpha)
\end{equation}
Thus, Equation~\ref{eqn:ABC2-4} is proved, showing the correctness of the algorithm.\\
%---------------------------


%---------------------------
From Lemmas~\ref{lem:rctr-1}, the total communication cost $M$ is
\[
M = O\left( \sqrt{p} \cdot \left( \sum_{k=1}^K \frac{d \cdot \log C_k^{max} }{\eps} + \sum_{i,j,k} \frac{\sqrt{d} \cdot \log C_{ijk}^{max} }{\eps} \right) \right)
\]
where $C_k^{max}$ and $C_{ijk}^{max}$ are the maximum values of the counters $C_k$ and $C_{ijk}$. Define $C^{max}$ as the total number of training instances, use the fact that $C_{ijk}^{max} < C_k^{max} < C^{max}$, $M$ can be written as
\[
M = O \left( \sqrt{p} \cdot \frac{d^{3/2}JK}{\eps} \log C^{max} \right)
\]

The size of our model is $O(dJK \log C^{max})$ bits and the local state requires total $O(pdJK \log C^{max})$ bits.
%---------------------------
\end{proof}
%----------------------------------



%-------------------------------------------------------------
\subsection{Varying Range of Possible Values Along Dimensions}
In the previous section, we assume different dimensions are having the same range of possible values $1,2, \cdots, J$, so we study the general case where each dimension has its own range of possible values and we suppose this range is already known in advance. For every $i \in [d]$, let attribute $X_i$ take on $J_i$ possible values $1,2, \cdots, J_i$, given value $j \in [J_i]$ and class label $k \in [K]$, let $\eps_i$ be the approximation factor of the distributed counter $\dc_{ijk}$ in Algorithm~\ref{algo:ABC2-init}. From the proof of Theorem~\ref{theo:ABC2-perf}, to achieve $\eps$-Approximate Bayesian Classifier, for any input vector $\alpha$, define $F=\prod_{i=1}^d \tilde{C}_{i\alpha_ik}$ and $f=\prod_{i=1}^d C_{i\alpha_ik}$, we should have
\begin{equation}
\var{F} \leq \frac{\eps^2 f^2}{128}
\end{equation}

With approximate factor $\eps_i$ for each dimension $i$, we can rewrite $\var{F}$ as
\begin{equation}
\var{F} \leq f^2 \cdot \left( \prod_{i=1}^d (1+\eps_i^2) \right) - f^2 \leq 2f^2 \cdot \sum_{i=1}^d \eps_i^2
\end{equation} 

On the other hand, the communication cost to maintain distributed counters $\dc_{ijk}$ is 
$O \left( \sqrt{p} K \log C^{max} \sum_{i=1}^d \frac{J_i}{\eps_i} \right)$. So our objective is given $0<\eps \leq 1/4$ and positive integers $J_1,J_2 \cdots J_d$, find the solution of $\eps_1, \eps_2, \cdots \eps_d$ such that
\begin{equation}
\label{eqn:restrict}
\begin{split}
\text{Minimize} \sum_{i=1}^d \frac{J_i}{\eps_i} \\
s.t. \quad \sum_{i=1}^d \eps_i^2 = \frac{\eps^2}{256}
\end{split}
\end{equation} 

\begin{claim}
The optimal solution of Equation~\ref{eqn:restrict} is 
\[
\eps_i = \frac{\eps \cdot J_i^{1/3}}{16 \cdot \left( \sum_{i=1}^d J_i^{2/3} \right)^{1/2}} \quad \quad i=1,2, \cdots, d
\]
\end{claim}
\begin{proof}
Use the Lagrange Multiplier to find the optimal solution, define the Lagrange function
\[
\mathcal{L} = \sum_{i=1}^d \frac{J_i}{\eps_i} + \lambda \left( \sum_{i=1}^d \eps_i^2 - \frac{\eps^2}{256} \right)
\]
We need to solve the equation set
\begin{equation}
\left\{
  \begin{array}{l}
  \frac{\partial \mathcal{L}}{\partial \eps_1} = -\frac{J_1}{\eps_1^2} + 2\lambda\eps_1 = 0 \\
  \frac{\partial \mathcal{L}}{\partial \eps_2} = -\frac{J_2}{\eps_2^2} + 2\lambda\eps_2 = 0 \\  
  \quad \quad \vdots  \\
  \frac{\partial \mathcal{L}}{\partial \eps_d} = -\frac{J_d}{\eps_d^2} + 2\lambda\eps_d = 0 \\ 
  \sum_{i=1}^d \eps_i^2 = \frac{\eps^2}{256}\\
  \end{array}
\right.
\end{equation}
There exists a unique solution $\eps_i = \frac{\eps \cdot J_i^{1/3}}{16 \cdot \left( \sum_{i=1}^d J_i^{2/3} \right)^{1/2}}$ for every $i \in [d]$, with which $\sum_{i=1}^d \frac{J_i}{\eps_i}$ can obtain the minima. 
The communication cost is 
\[
M = O \left( \sqrt{p} K \cdot \frac{\left( \sum_{i=1}^d J_i^{2/3} \right)^{3/2}}{\eps} \log C^{max} \right)
\]
\end{proof}




